DiffSim: Taming Diffusion Models for Evaluating Visual Similarity

Diffusion models have fundamentally transformed the field of generative models, making the assessment of similarity between customized model outputs and reference inputs critically important. However, traditional perceptual similarity metrics operate primarily at the pixel and patch levels, comparing low-level colors and textures but failing to capture mid-level similarities and differences in image layout, object pose, and semantic content. Contrastive learning-based CLIP and self-supervised learning-based DINO are often used to measure semantic similarity, but they highly compress image features, inadequately assessing appearance details. This paper is the first to discover that pretrained diffusion models can be utilized for measuring visual similarity and introduces the DiffSim method, addressing the limitations of traditional metrics in capturing perceptual consistency in custom generation tasks. By aligning features in the attention layers of the denoising U-Net, DiffSim evaluates both appearance and style similarity, showing superior alignment with human visual preferences. Additionally, we introduce the Sref and IP benchmarks to evaluate visual similarity at the level of style and instance, respectively. Comprehensive evaluations across multiple benchmarks demonstrate that DiffSim achieves state-of-the-art performance, providing a robust tool for measuring visual coherence in generative models.

==> sec/2_method_old.tex <==
\begin{table}[ht]
\centering
\caption{Evaluation of Different DiffSim Architectures.}
\label{tab:diffsim_setting}
\setlength{\tabcolsep}{4pt}
\footnotesize 
\begin{tabular}{@{}lccc@{}}
\toprule
DiffSim Setting & DiffSim SD1.5 & DiffSim-IPA SD1.5 & DiffSim SD-XL \\ \midrule
Sref       & \textbf{97.40\%} & 94.70\% & 93.05\% \\
IP      & \textbf{92.04\%} & 77.06\% & 83.41\% \\
NIGHTS      & \textbf{86.82\%} & 79.16\% & 78.05\% \\
CUTE      & 72.06\%  & \textbf{76.17\%} & 69.94\% \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Performance of Different Metrics on Tiktok Dataset.}
\label{tab:tiktok}
\setlength{\tabcolsep}{4pt}
\footnotesize 
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Metrics} & LPIPS & CLIP & DINO v2 & FFA \\ \midrule
Variance $\downarrow$ & 3.565e-3 & 1.007e-3 & 6.340e-3 & 4.381e-3\\
\midrule
\textbf{Metrics} & CLIP AAS & DINO v2 AAS & DiffSim \\ \midrule
Variance $\downarrow$ & 4.397e-7 & 1.825e-3 & 1.335e-3 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table*}[ht]
\centering
\caption{Performance of Different Metrics across Various Benchmarks.}
\label{tab:performance}
\small 
\begin{tabular}{@{}c|cc|cc|c|cc@{}}
\toprule
\textbf{Model / Benchmark} & \multicolumn{2}{c|}{\textbf{Human-align Similarity}} & \multicolumn{2}{c|}{\textbf{Instance Similarity}} & \multicolumn{1}{c|}{\textbf{Low-level Similarity}} & \multicolumn{2}{c}{\textbf{Style Similarity}} \\ 
 & \textbf{NIGHTSS} & \textbf{Dreambench++} & \textbf{CUTE} & \textbf{IP} & \textbf{TID2013} & \textbf{Sref}  & \textbf{InstantStyle bench} \\ \midrule
LPIPS\cite{lpips}                     & 71.13\%           & 62.33\%                  & 63.17\%          & 84.01\%          & 94.50\%           & 87.85\%                           & 93.15\%  \\
Gram \cite{}                      & -           & -                  & -          & -          & -           & 84.05\%                          & 88.30\%  \\
CLIP \cite{clip}                      & 82.26\%           & 70.54\%                  & 72.71\%          & 91.70\%          & 90.33\%           & 84.60\%                           & 82.90\%  \\
DINO v2 \cite{dinov2}                   & 85.24\%           & 72.25\%                  & 77.27\%          & 85.35\%          & 91.50\%           & 87.20\%                           & 86.10\%  \\
FFA \cite{apple}                       & 77.78\%           & 65.21\%                  & 76.55\%          & 89.70\%          & 75.17\%           & 62.15\%                            & 62.90\%  \\
CLIP AAS (ours)               & X\%           & 67.23\%                  & 71.78\%          & 88.03\%          & 96.33\%           & 75.85\%                            & X\%  \\
DINO v2 AAS (ours)              &68.3\%           & 70.01\%                  & 77.04\%          & 89.77\%          & 95.83\%           & 73.39\%                          & 81.30\%  \\
DiffSim (ours)                   & 86.82\%           & 72.04\%                  & 76.17\%          & 92.04\%          & 94.17\%           & 97.40\%                         & 96.60\%  \\ \bottomrule
\end{tabular}
\end{table*}


\subsubsection{DiffSim in cross-attn block}
% SD Unet通过在其交叉注意力层中整合文本嵌入作为条件，实现了文本到图像的生成。之前的研究如Custom Diffusion已经指出这些交叉注意力层在学习定制化模型概念中的关键作用，显示出仅通过微调这些层就能实现新概念的学习。因此我们自然的想到在用交叉层的特征评估图像相似性， 然而交叉注意力层仅支持图像latent和text embedding计算交叉注意力。为此，我们求助于IP-Adapter Plus， IP-Adapter Plus采用了CLIP图像编码器的补丁特征，并将IP token数目增加到16，将IP token注入Unet的交叉注意力层。我们设计了如图2（c)中的结构，图A和图B分别作为IP-Adapter Plus和去噪Unet的输入，计算AAS（L_B,L_A), 然后交换两张图的输入位置，计算AAS（L_A,L_B). 图A和图B的相似性被定义为：

The SD Unet enhances text-to-image generation by integrating text embeddings as conditions within its cross-attention layers. Prior studies like Custom Diffusion have highlighted the pivotal role of these layers in learning customized model concepts, demonstrating that new concepts can be learned through mere fine-tuning of these layers. This naturally led us to consider using features from cross-attention layers to assess image similarity; however, cross-attention layers only support the calculation of attention between image latents and text embeddings. To address this, we turn to IP-Adapter Plus. IP-Adapter Plus utilizes patch features from the CLIP image encoder and increases the number of IP tokens to 16, injecting these tokens into the cross-attention layers of Unet. We designed the structure shown in Figure 2(c), where Image \(I_A\) and Image \(I_B\) are fed into IP-Adapter Plus and the denoising Unet, respectively, to compute \(\text{AAS}(L_B, L_A)\), then swap the inputs of the two images and compute \(\text{AAS}(L_A, L_B)\). The similarity between Image \(I_A\) and \(I_B\) is defined as:
\begin{equation}
\begin{aligned}
\text{DiffSim}(I_A, I_B, n, t) &= \frac{1}{2} \left( \text{AAS}(L_A^{\text{cross}, n, t}, L_B^{\text{cross}, n, t}) \right. \\
&\quad \left. + \text{AAS}(L_B^{\text{cross}, n, t}, L_A^{\text{cross}, n, t}) \right)
\end{aligned}
\end{equation}
where \(L_A^{cross, n, t}\) and \(L_B^{cross, n, t}\) denote the latent representations of images \(I_A\) and \(I_B\) within the \(n\)-th cross-attention layer of the U-Net at denoising timestep \(t\), respectively.


\subsection{Aligned Attention Score}
In this section, we introduce the Aligned Attention Score (AAS), a novel metric designed to evaluate the similarity between two images by comparing their features using attention mechanisms within a neural network. This method employs the attention layers of a pre-trained U-Net or other Transformer-based models, processing the feature vectors of images \(I_A\) and \(I_B\) through attention functions to generate aligned representations. 

We define \(L_A\) and \(L_B\) as the latent representations of images \(I_A\) and \(I_B\), respectively. In our implementation, the attention function $\text{attn}(Q, K, V)$ aligns these latents by computing the similarity score using the query (\(Q\)), key (\(K\)), and value (\(V\)) matrices derived from \(L_A\) and \(L_B\). Specifically, we calculate:
\begin{align}
    \text{AAS}(L_A, L_B) &= \cos(\text{attn}(Q_A, K_A, V_A), \notag \\
    &\quad \text{attn}(Q_A, K_B, V_B)) \\
    \text{AAS}(L_B, L_A) &= \cos(\text{attn}(Q_B, K_B, V_B), \notag \\
    &\quad \text{attn}(Q_B, K_A, V_A))
\end{align}
and the overall similarity of \(L_A\) and \(L_B\) can be defined as:
\begin{align}
\text{Similarity}(L_A, L_B) &= \text{AAS}(L_A, L_B) + \text{AAS}(L_B, L_A)
\end{align}



This dual computation ensures that each image's features are evaluated both as queries and as keys against the other's features, providing a robust measure of visual similarity.

The AAS metric excels in tasks where traditional metrics fall short, particularly in handling variations in style, pose, and context between images. By focusing on feature alignment rather than direct pixel comparison, AAS can more accurately reflect perceptual similarities as understood by human observers.



\section{Method}
%本节我介绍DiffSim的方法。 3.1节介绍包括扩散模型和Stable diffusion model 中的注意力机制作为前置知识。 3.2节介绍DiffSim核心实现方法 3.3节介绍如何在不同模型架构上实现DiffSim，扩散稳定扩散模型、CLIP、DINO。

In this section, I introduce the methodology of DiffSim. Section 3.1 presents the foundational knowledge, including the diffusion model and attention mechanisms in the Stable Diffusion model. Section 3.2 details the core implementation of DiffSim. Section 3.3 describes how to implement DiffSim across different model architectures: Stable Diffusion, CLIP, and DINO.


\subsection{Preliminaries}
\subsubsection{Diffusion Model}

Diffusion models \cite{sohl2015deep, ho2020denoising} are designed to convert a Normal distribution into an arbitrary data distribution, applied here over 2D image spaces.

In training, we add Gaussian noise of increasing magnitude to clean images \( x_0 \) from the dataset to generate noisy versions \( x_t \), modeled by:
\begin{equation}
x_t = \sqrt{\alpha_t} x_0 + \sqrt{1 - \alpha_t} \epsilon,
\end{equation}
where \( \epsilon \sim \mathcal{N}(0, I) \) represents the noise sampled randomly and \( t \) denotes the time steps in the diffusion sequence with \( \alpha_t \) controlling the noise level.

The network \( f_{\theta} \), often a U-Net \cite{ronneberger2015u, ronneberger2019tensorized}, predicts noise \( \epsilon \) from \( x_t \) and \( t \). It iteratively denoises starting from \( x_T \), purely noise, back to \( x_0 \), reconstructing the original image from distorted data.



%扩散模型\cite{sohl2015deep, ho2020denoising}旨在将正态分布转换为任意数据分布，本文中应用于二维图像空间。

%在训练过程中，我们将不同强度的高斯噪声添加到干净的图像\( x_0 \)中，生成噪声图像\( x_t \)，通过以下模型表示：
%\begin{equation}
%x_t = \sqrt{\alpha_t} x_0 + \sqrt{1 - \alpha_t} \epsilon, \end{equation}
%其中\( \epsilon \sim \mathcal{N}(0, I) \)代表随机采样的噪声，\( t \)表示扩散过程中的时间步长，\( \alpha_t \)控制噪声水平。网络\( f_{\theta} \)，通常为U-Net\cite{ronneberger2015u, ronneberger2019tensorized}，从\( x_t \)和\( t \)预测输入噪声\( \epsilon \)。它从纯噪声\( x_T \)开始迭代去噪，最终从扰动数据中重建原始图像。



\subsubsection{Attention mechanisms in stable diffusion}
In this section, we analyze how cross and self-attention maps in Stable Diffusion contribute to the effectiveness of DiffSim.

%在稳定扩散和其他类似模型中，交叉注意力层在融合图像和文本中起到关键作用，使 T2I 模型能够生成与文本描述一致的图像。如图2上部所示，交叉注意力层从噪声图像和提示中接收查询矩阵、键矩阵和值矩阵，即 $Q_{\text{cross}}$、$K_{\text{cross}}$ 和 $V_{\text{cross}}$。具体来说，$Q_{\text{cross}}$ 是通过学习的线性投影 $\ell_q$ 从噪声图像的空间特征 $\phi_{\text{cross}}(z_t)$ 中得到的，而 $K_{\text{cross}}$ 和 $V_{\text{cross}}$ 是使用学习的线性投影 $\ell_k$ 和 $\ell_v$ 从输入提示 $P$ 的文本嵌入 $P_{\text{emb}}$ 中投影得到的。交叉注意力图定义如下： \begin{align} Q_{\text{cross}} &= \ell_q(\phi_{\text{cross}}(z_t)), \ K_{\text{cross}} &= \ell_k(P_{\text{emb}}), \ M_{\text{cross}} &= \text{Softmax}\left(\frac{Q_{\text{cross}} K_{\text{cross}}^T}{\sqrt{d_{\text{cross}}}}\right), \end{align} 其中 $d_{\text{cross}}$ 是键和查询的维度。最终输出定义为文本和图像的融合特征，表示为 $\hat{\phi}(z_t) = M_{\text{cross}} V_{\text{cross}}$，其中 $V_{\text{cross}} = \ell_v(P_{\text{emb}})$。直观上，交叉注意力图中的每个单元 $M_{ij}$ 决定了分配给图像中第 $i$ 个空间特征相对于第 $j$ 个标记的值的权重。交叉注意力图使扩散模型能够在图像区域定位/对齐提示的标记。
\textbf{Cross attention.} In Stable Diffusion and other similar models, cross-attention layers play a crucial role in fusing images and texts, allowing T2I models to generate images that are consistent with textual descriptions. As depicted in the upper part of Figure ~\ref{fig:method}, the cross-attention layer receives the query, key, and value matrices, i.e., $Q_{\text{cross}}$, $K_{\text{cross}}$, and $V_{\text{cross}}$, from the noisy image and prompt. Specifically, $Q_{\text{cross}}$ is derived from the spatial features of the noisy image $\phi_{\text{cross}}(z_t)$ by learned linear projections $\ell_q$, while $K_{\text{cross}}$ and $V_{\text{cross}}$ are projected from the textual embedding $P_{\text{emb}}$ of the input prompt $P$ using learned linear projections denoted as $\ell_k$ and $\ell_v$, respectively. The cross-attention map is defined as:
\begin{align}
Q_{\text{cross}} &= \ell_q(\phi_{\text{cross}}(z_t)), \\
K_{\text{cross}} &= \ell_k(P_{\text{emb}}), \\
M_{\text{cross}} &= \text{Softmax}\left(\frac{Q_{\text{cross}} K_{\text{cross}}^T}{\sqrt{d_{\text{cross}}}}\right),
\end{align}
where $d_{\text{cross}}$ is the dimension of the keys and queries. The final output is defined as the fused feature of the text and image, denoted as $\hat{\phi}(z_t) = M_{\text{cross}} V_{\text{cross}}$, where $V_{\text{cross}} = \ell_v(P_{\text{emb}})$. Intuitively, each cell in the cross-attention map, denoted as $M_{ij}$, determines the weights attributed to the value of the $j$-th token relative to the spatial feature $i$ of the image. The cross-attention map enables the diffusion model to locate/align the tokens of the prompt in the image area.

% 如图2所示，与交叉注意力不同，自注意力层通过学习的线性投影 $\bar{\ell}K$ 和 $\bar{\ell}Q$ 分别从噪声图像 $\phi{\text{self}} (z_t)$ 接收键矩阵 $K{\text{self}}$ 和查询矩阵 $Q_{\text{self}}$。自注意力图定义如下： \begin{align} Q_{\text{self}} &= \bar{\ell}q(\phi{\text{self}} (z_t)), \ K_{\text{self}} &= \bar{\ell}K(\phi{\text{self}} (z_t)), \ M_{\text{self}} &= \text{Softmax}\left(\frac{Q_{\text{self}} K_{\text{self}}^T}{\sqrt{d_{\text{self}}}}\right), \end{align} 其中 $d_{\text{self}}$ 是 $K_{\text{self}}$ 和 $Q_{\text{self}}$ 的维度。$M_{\text{self}}$ 决定了分配给图像中第 $i$ 和第 $j$ 个空间特征相关性的权重，并且可以影响生成图像的空间布局和形状细节。因此，自注意力图可以用来在图像编辑过程中保持原始图像的空间结构特征
\textbf{Self attention.} As depicted in Figure ~\ref{fig:method}, unlike cross-attention, the self-attention layer receives the keys matrix $K_{\text{self}}$ and the query matrix $Q_{\text{self}}$ from the noisy image $\phi_{\text{self}} (z_t)$ through learned linear projections $\bar{\ell}_K$ and $\bar{\ell}_Q$, respectively. The self-attention map is defined as:
\begin{align}
Q_{\text{self}} &= \bar{\ell}_q(\phi_{\text{self}} (z_t)), \\
K_{\text{self}} &= \bar{\ell}_K(\phi_{\text{self}} (z_t)), \\
M_{\text{self}} &= \text{Softmax}\left(\frac{Q_{\text{self}} K_{\text{self}}^T}{\sqrt{d_{\text{self}}}}\right),
\end{align}
where $d_{\text{self}}$ is the dimension of $K_{\text{self}}$ and $Q_{\text{self}}$. $M_{\text{self}}$ determines the weights assigned to the relevance of the $i$-th and $j$-th spatial features in the image and can affect the spatial layout and shape details of the generated image. Consequently, the self-attention map can be utilized to preserve the spatial structure characteristics of the original image throughout the image editing process.


\subsection{Feature Alignment Attention Index}
The Feature Alignment Attention Index (FAAI) is a novel metric developed to evaluate the similarity between two images by dynamically comparing their features using attention mechanisms within a neural network. This method leverages the cross-attention layers of a pre-trained U-Net, where the feature vectors of images \(I_A\) and \(I_B\) are processed through attention functions to generate aligned representations.

In our implementation, the attention function $\text{attn}(Q, K, V)$ computes the similarity score by aligning the query $(Q)$, key $(K)$, and value $(V)$ matrices derived from the respective images. Specifically, we perform the following operations:
\begin{align*}
\text{Similarity}(I_A, I_B) &= \cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_B, K_B, V_B)) \\
&+ \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_A, K_A, V_A)).
\end{align*}
This dual computation ensures that each image's features are evaluated both as queries and as keys against the other's features, thus providing a robust measure of visual similarity.

The FAAI metric excels in tasks where traditional metrics fall short, particularly in handling variations in style, pose, and context between the images being compared. By focusing on feature alignment rather than direct pixel comparison, FAAI can more accurately reflect perceptual similarities as understood by human observers. This metric has proven particularly effective in applications requiring fine-grained analysis of image content and style, such as style transfer validation, historical image analysis, and synthetic image detection.


\subsection{Diff-SIM in self-attn}
% 在海量图像文本对上预训练的stable diffusion unet是出色的视觉特征提取器，reference only方法直接将参考图像输入unet并将自注意力层中参考图的K和V直接与去噪unet的自注意力层中的K和V相连，实现了一致性的图像variation。 类似的，人体驱动任务中animate anyone, magicanimate等将unet作为提取参考图像细节信息的ReferenceNet, 并将ReferenceNet和去噪Unet的自注意力层相连进行条件信息的注入。同样的做法还被应用于人脸驱动和和Image2Video 。

% 在上述方法中，自注意力层中特征的嵌入可以实现外观一致性的图像或视频的生成，因此我们认为unet自注意力层的特征可以反应图像外观的一致性。我们提出了DiffSim的自注意力层实现， 对于图像I_{A}和图像I_{B}，在Unet的某一个自注意力层中的Q，K， V分别是Q_{A}, K_{A}, V_{A}和Q_{B}, K_{B}, V_{B}, 图像相似性分数被定义为：Similarity(I_{A},I_{B} = cos(attn(Q_{A}, K_{A}, V_{A}), attn(Q_{A}, K_{B}, V_{B}) + cos(attn(Q_{B}, K_{B}, V_{B}), attn(Q_{B}, K_{A}, V_{A})

% 在自注意力层中，图A和图B的latent在空间上不是pixel align的，所以不能直接逐像素计算A和B latent的距离。为此，我们使用注意力操作将A和B对齐，在自注意力层中attn(Q_{A}, K_{A}, V_{A}), attn(Q_{A}, K_{B}, V_{B}是对齐的。

The pre-trained Stable Diffusion U-Net, extensively trained on massive image-text pairs, excels as a visual feature extractor. The reference only\citep{referenceonly} approach inputs reference images directly into the U-Net, connecting the reference image's keys (K) and values (V) in the self-attention layers directly with those in the denoising U-Net's self-attention layers to achieve consistent image variations. Similarly, in human-driven tasks such as Animate Anyone and MagicAnimate\citep{magicanimate, animateanyone}, the U-Net serves as a ReferenceNet to extract detailed information from reference images, linking its self-attention layers with those of the denoising U-Net for injecting conditional information. This technique is also applied in face-driven tasks\citep{emo, echomimic, idanimator, x-portrait}, image customization generation \citep{referenceonly, stablemakeup, stablehair}, and Image2Video generation \citep{livephoto, i2vgen-xl}. 

In the aforementioned methods, the embedding of features in the self-attention layers enables the generation of images or videos with appearance consistency. Thus, we posit that the features in the U-Net's self-attention layers can reflect the consistency of image appearance. We propose an implementation of the self-attention layers in DiffSim. In the self-attention layer, the latent representations of Image A and Image B are not spatially pixel-aligned. Consequently, it is not feasible to directly compute the distances between the latents of A and B on a pixel-by-pixel basis. To overcome this, we utilize an attention mechanism to align A and B, where the alignment operations are $\text{attn}(Q_A, K_A, V_A)$ and $\text{attn}(Q_A, K_B, V_B)$. These functions ensure that the representations of both images are aligned, allowing for more accurate comparative and analytical operations. For images \(I_A\) and \(I_B\), within a certain self-attention layer of U-Net, \(Q\), \(K\), \(V\) are \(Q_A\), \(K_A\), \(V_A\) and \(Q_B\), \(K_B\), \(V_B\) respectively. The image similarity score is defined as:
\begin{align*}
\text{Similarity}(I_A, I_B) &= \\
\quad &\cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_B, K_B, V_B)) \\
\quad &+ \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_A, K_A, V_A)).
\end{align*}


\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{sec/Image/Sref.png}
    \caption{Some examples in Sref benchmark we selected. Midjourney's style references allow users to guide the aesthetics and style of the images generated by using external pictures or sref seeds in prompts. We have curated a collection of 508 styles on internet, each handpicked by human artists and represented by four different thematic reference images.}
    \label{fig:art}
\end{figure*}


\subsection{Diff-SIM in cross-attn}
% SD Unet通过在其交叉注意力层中整合文本嵌入作为条件，增强了文本到图像的生成。之前的研究如Custom Diffusion已经指出这些交叉注意力层在学习定制化模型概念中的关键作用，显示出仅通过微调这些层就能实现定制化生成。IP-Adapter扩展了这一概念，通过Adapter将CLIP image feature注入Unet的交叉注意力层，而无需广泛重训练。IP-Adapter Plus则更进一步，采用了CLIP图像编码器的补丁特征，并将IP token数据增加到16，显著提高了生成结果与参考图像之间的一致性，从而改善了模型根据特定文本描述和视觉上下文更精确地对齐生成内容的能力。

% 与DiffSim的自注意力版本实现不同，我们分别将图像A和图像B输入IP-Adapter Plus分支和去噪Unet，并在unet的交叉注意力层计算attn(Q_{A}, K_{A}, V_{A}), attn(Q_{A}, K_{B}, V_{B}, 然后我们交换图A和图B的位置，计算attn(Q_{B}, K_{A}, V_{A}) 和 attn(Q_{B}, K_{B}, V_{B}). 图A和图B的相似性被定义为：
% \begin{align*}
% \text{Similarity}(I_A, I_B) &= \\
% \quad &\cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_B, K_B, V_B)) \\
% \quad &+ \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_A, K_A, V_A)).
% \end{align*}



SD Unet enhances text-to-image generation by integrating text embeddings as conditions within its cross-attention layers. Previous research such as Custom Diffusion has highlighted the critical role of these cross-attention layers in learning customized model concepts, demonstrating that tailored generation can be achieved by merely fine-tuning these layers. The IP-Adapter extends this concept by using an adapter to inject CLIP image features into the cross-attention layers of Unet, without the need for extensive retraining. IP-Adapter Plus goes even further by utilizing patch features from the CLIP image encoder and increasing the IP token data to 16, significantly enhancing the consistency between generated results and reference images. This improvement enables the model to more precisely align generated content with specific textual descriptions and visual contexts. 


Unlike the self-attention version of DiffSim, for this approach, we input images \(I_A\) and \(I_B\) into the IP-Adapter Plus and the denoising U-Net. We perform calculations within the U-Net's cross-attention layers, where the attention functions \(\text{attn}(Q_A, K_A, V_A)\) and \(\text{attn}(Q_A, K_B, V_B)\) are first computed. After swapping the positions of \(I_A\) and \(I_B\), the functions \(\text{attn}(Q_B, K_A, V_A)\) and \(\text{attn}(Q_B, K_B, V_B)\) are computed. The similarity between the two images is then defined as:
\begin{align*}
\text{Similarity}(I_A, I_B) &= \\
\quad &\cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_B, K_B, V_B)) \\
\quad &+ \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_A, K_A, V_A)).
\end{align*}
This method enhances the capability to accurately assess perceptual similarities between the two images by dynamically comparing features under varying conditions.

\subsection{Extend DiffSim to other frameworks}
% DiffSim的方法具有广泛的适用性，可以通过计算注意力层中特征相似性来分析两张图像的特征。我们已将DiffSim方法扩展应用于CLIP Image Encoder和DINO v2架构。CLIP通过对比学习训练图像和文本编码器，以理解图像与文本之间的关系，并最大化匹配图文对的相似性，通常采用Vision Transformer或ResNet作为图像编码器。DINO采用自监督方式，通过教师-学生网络架构，其中两者均使用Vision Transformer，学生网络通过模仿经数据增强的输入和教师网络的输出来学习视觉表示，教师网络则通过指数移动平均（EMA）进行更新。在特定自注意力层上，我们计算图像相似度，开发了新的指标CLIP Cross-SiM和DINO v2 Cross-Sim来评估相似性。

The DiffSim method is widely applicable and allows for the analysis of image features by computing feature similarity in the attention layers. We have extended the DiffSim approach to the CLIP Image Encoder and DINO v2 architectures. CLIP trains image and text encoders through contrastive learning to understand the relationship between images and text, aiming to maximize the similarity of matching image-text pairs, typically using Vision Transformer or ResNet as the image encoder. DINO operates in a self-supervised manner with a teacher-student network architecture, both utilizing Vision Transformers. The student network learns visual representations by mimicking the output of the teacher network, which has been augmented with random data transformations. The teacher network is updated through exponential moving average (EMA). On specific self-attention layers, we calculate image similarity and have developed new metrics, CLIP Cross-Sim and DINO v2 Cross-Sim, to assess this similarity.

==> sec/2_method_old2.tex <==
\vspace{-0.5em}
\section{Method}
%本节我介绍DiffSim的方法。 3.1节介绍包括扩散模型和Stable diffusion model 中的注意力机制作为前置知识。 3.2节介绍DiffSim核心实现方法 3.3节介绍如何在不同模型架构上实现DiffSim，扩散稳定扩散模型、CLIP、DINO。

 Section Sec. \ref{sec:1} presents attention mechanisms in the Stable Diffusion model. Sec. \ref{sec:2} introduce Aligned Attention Score we proposed. Sec. \ref{sec:3} describes how to implement DiffSim across different model architectures. Sec. \ref{sec:4} introduce two benchmark we propose.

\vspace{-0.3em}
\subsection{Preliminaries}
\label{sec:1}
% In this section, we introduce attention mechanisms in stable diffusion.

% \subsubsection{Diffusion Model}
%Diffusion models \cite{sohl2015deep, ho2020denoising} are designed to convert a Normal distribution into an arbitrary data distribution, applied here over 2D image spaces. In training, add Gaussian noise of increasing magnitude to clean images \( x_0 \) from the dataset to generate noisy versions \( x_t \), modeled by:
%\begin{equation}
%x_t = \sqrt{\alpha_t} x_0 + \sqrt{1 - \alpha_t} \epsilon,
%\end{equation}
%where \( \epsilon \sim \mathcal{N}(0, I) \) represents the noise sampled randomly and \( t \) denotes the time steps in the diffusion sequence with \( \alpha_t \) controlling the noise level. The network \( f_{\theta} \), often a U-Net \cite{ldm}, predicts noise \( \epsilon \) from \( x_t \) and \( t \). It iteratively denoises starting from \( x_T \), purely noise, back to \( x_0 \), reconstructing the original image from distorted data.



%扩散模型\cite{sohl2015deep, ho2020denoising}旨在将正态分布转换为任意数据分布，本文中应用于二维图像空间。

%在训练过程中，我们将不同强度的高斯噪声添加到干净的图像\( x_0 \)中，生成噪声图像\( x_t \)，通过以下模型表示：
%\begin{equation}
%x_t = \sqrt{\alpha_t} x_0 + \sqrt{1 - \alpha_t} \epsilon, \end{equation}
%其中\( \epsilon \sim \mathcal{N}(0, I) \)代表随机采样的噪声，\( t \)表示扩散过程中的时间步长，\( \alpha_t \)控制噪声水平。网络\( f_{\theta} \)，通常为U-Net\cite{ronneberger2015u, ronneberger2019tensorized}，从\( x_t \)和\( t \)预测输入噪声\( \epsilon \)。它从纯噪声\( x_T \)开始迭代去噪，最终从扰动数据中重建原始图像。


%在稳定扩散和其他类似模型中，交叉注意力层在融合图像和文本中起到关键作用，使 T2I 模型能够生成与文本描述一致的图像。如图2上部所示，交叉注意力层从噪声图像和提示中接收查询矩阵、键矩阵和值矩阵，即 $Q_{\text{cross}}$、$K_{\text{cross}}$ 和 $V_{\text{cross}}$。具体来说，$Q_{\text{cross}}$ 是通过学习的线性投影 $\ell_q$ 从噪声图像的空间特征 $\phi_{\text{cross}}(z_t)$ 中得到的，而 $K_{\text{cross}}$ 和 $V_{\text{cross}}$ 是使用学习的线性投影 $\ell_k$ 和 $\ell_v$ 从输入提示 $P$ 的文本嵌入 $P_{\text{emb}}$ 中投影得到的。交叉注意力图定义如下： \begin{align} Q_{\text{cross}} &= \ell_q(\phi_{\text{cross}}(z_t)), \ K_{\text{cross}} &= \ell_k(P_{\text{emb}}), \ M_{\text{cross}} &= \text{Softmax}\left(\frac{Q_{\text{cross}} K_{\text{cross}}^T}{\sqrt{d_{\text{cross}}}}\right), \end{align} 其中 $d_{\text{cross}}$ 是键和查询的维度。最终输出定义为文本和图像的融合特征，表示为 $\hat{\phi}(z_t) = M_{\text{cross}} V_{\text{cross}}$，其中 $V_{\text{cross}} = \ell_v(P_{\text{emb}})$。直观上，交叉注意力图中的每个单元 $M_{ij}$ 决定了分配给图像中第 $i$ 个空间特征相对于第 $j$ 个标记的值的权重。交叉注意力图使扩散模型能够在图像区域定位/对齐提示的标记。

\subsubsection{Cross Attention in Stable Diffusion} 
In Stable Diffusion and other similar models, cross-attention layers play a crucial role in fusing images and texts, allowing diffusion models to generate images that are consistent with textual descriptions. The cross-attention layer receives the query, key, and value matrices, i.e., $Q_{\text{cross}}$, $K_{\text{cross}}$, and $V_{\text{cross}}$, from the noisy image and prompt. Specifically, $Q_{\text{cross}}$ is derived from the spatial features of the noisy image $\phi_{\text{cross}}(z_t)$ by learned linear projections $\ell_q$, while $K_{\text{cross}}$ and $V_{\text{cross}}$ are projected from the textual embedding $P_{\text{emb}}$ of the input prompt $P$ using learned linear projections denoted as $\ell_k$ and $\ell_v$, respectively. The cross-attention map is defined as:
\begin{align}
Q_{\text{cross}} &= \ell_q(\phi_{\text{cross}}(z_t)), \\
K_{\text{cross}} &= \ell_k(P_{\text{emb}}), \\
M_{\text{cross}} &= \text{Softmax}\left(\frac{Q_{\text{cross}} K_{\text{cross}}^T}{\sqrt{d_{\text{cross}}}}\right),
\end{align}
where $d_{\text{cross}}$ is the dimension of the keys and queries. The final output is defined as the fused feature of the text and image, denoted as $\hat{\phi}(z_t) = M_{\text{cross}} V_{\text{cross}}$, where $V_{\text{cross}} = \ell_v(P_{\text{emb}})$. Intuitively, each cell in the cross-attention map, denoted as $M_{ij}$, determines the weights attributed to the value of the $j$-th token relative to the spatial feature $i$ of the image. The cross-attention map enables the diffusion model to locate/align the tokens of the prompt in the image area.

% 如图2所示，与交叉注意力不同，自注意力层通过学习的线性投影 $\bar{\ell}K$ 和 $\bar{\ell}Q$ 分别从噪声图像 $\phi{\text{self}} (z_t)$ 接收键矩阵 $K{\text{self}}$ 和查询矩阵 $Q_{\text{self}}$。自注意力图定义如下： \begin{align} Q_{\text{self}} &= \bar{\ell}q(\phi{\text{self}} (z_t)), \ K_{\text{self}} &= \bar{\ell}K(\phi{\text{self}} (z_t)), \ M_{\text{self}} &= \text{Softmax}\left(\frac{Q_{\text{self}} K_{\text{self}}^T}{\sqrt{d_{\text{self}}}}\right), \end{align} 其中 $d_{\text{self}}$ 是 $K_{\text{self}}$ 和 $Q_{\text{self}}$ 的维度。$M_{\text{self}}$ 决定了分配给图像中第 $i$ 和第 $j$ 个空间特征相关性的权重，并且可以影响生成图像的空间布局和形状细节。因此，自注意力图可以用来在图像编辑过程中保持原始图像的空间结构特征

\subsubsection{Self Attention in Stable Diffusion}  Unlike cross-attention, the self-attention layer receives the keys matrix $K_{\text{self}}$ and the query matrix $Q_{\text{self}}$ from the noisy image $\phi_{\text{self}} (z_t)$ through learned linear projections $\bar{\ell}_K$ and $\bar{\ell}_Q$, respectively. The self-attention map is defined as:
\begin{align}
Q_{\text{self}} &= \bar{\ell}_q(\phi_{\text{self}} (z_t)), \\
K_{\text{self}} &= \bar{\ell}_K(\phi_{\text{self}} (z_t)), \\
M_{\text{self}} &= \text{Softmax}\left(\frac{Q_{\text{self}} K_{\text{self}}^T}{\sqrt{d_{\text{self}}}}\right),
\end{align}
where $d_{\text{self}}$ is the dimension of $K_{\text{self}}$ and $Q_{\text{self}}$. $M_{\text{self}}$ determines the weights assigned to the relevance of the $i$-th and $j$-th spatial features in the image and can affect the spatial layout and shape details of the generated image. Consequently, the self-attention map can be utilized to preserve the spatial structure characteristics of the original image throughout the image editing process.


\vspace{-0.2em}
\subsection{Aligned Attention Score}
\vspace{-0.2em}
\label{sec:2}
In this section, we introduce the Aligned Attention Score (AAS), a novel metric designed to overcome the limitations of traditional similarity assessments like Mean Squared Error (MSE) or cosine similarity, which assume pixel-level alignment between images's latent. Such assumptions are often violated in real-world scenarios where images can exhibit significant variations in style, pose, or context, leading to ineffective and inaccurate similarity measurements.

Moreover, popular methods such as CLIP and DINO compress high-dimensional patch features into a low-dimensional feature space using Multilayer Perceptrons (MLPs), calculating cosine similarity on these reduced representations. While effective for semantic-level comparisons, this compression leads to a substantial loss of detailed information, failing to capture finer nuances that are critical for certain applications.

We define \(L_A\) and \(L_B\) as the latent representations of images \(I_A\) and \(I_B\), respectively. To address the misalignment and information loss issues, our implementation employs the attention function $\text{attn}(Q, K, V)$ within a neural network to dynamically align these representations:
\vspace{-0.5em}
\begin{align}
    \text{AAS}(L_A, L_B) &= \cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_A, K_B, V_B)), \\
    \text{AAS}(L_B, L_A) &= \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_B, K_A, V_A)).
\end{align}
By processing the features through attention mechanisms in pre-trained U-Net or Transformer-based models, AAS aligns two dense latents in the attention layers, ensuring that each image's features are evaluated both as queries and as keys against the other's features, thereby providing a robust measure of visual similarity:
\vspace{-0.5em}
\begin{equation}
\text{Similarity}(L_A, L_B) = \frac{1}{2} \left(  \text{AAS}(L_A, L_B) + \text{AAS}(L_B, L_A) \right).
\end{equation}
This method not only compensates for the lack of pixel alignment but also preserves the richness of the feature space, offering a more accurate reflection of perceptual similarities that align closely with human visual judgment. 


%subsection{对齐注意力分数}在本节中，我们介绍了对齐注意力分数（AAS），这是一种旨在克服传统相似性评估（如均方误差（MSE）或余弦相似度）的局限性的新指标。这些传统方法假设图像潜在特征之间在像素层面上是对齐的，但在实际应用中，图像常常因风格、姿态或上下文的显著变化而违反这一假设，导致相似性测量的效果不佳和不准确。此外，如CLIP和DINO等流行方法通过多层感知机（MLPs）将高维块特征压缩到低维特征空间，并在这些简化的表征上计算余弦相似度。尽管这种方法在语义级比较上有效，但压缩过程会导致大量细节信息的丢失，未能捕捉到某些应用中至关重要的微妙差别。我们定义 \(L_A\) 和 \(L_B\) 分别为图像 \(I_A\) 和 \(I_B\) 的潜在表征。为了解决错位和信息丢失的问题，我们的实现通过神经网络中的注意力函数 $\text{attn}(Q, K, V)$ 动态对齐这些表征：\begin{align}   \text{AAS}(L_A, L_B) &= \cos(\text{attn}(Q_A, K_A, V_A), \text{attn}(Q_A, K_B, V_B)) \\\text{AAS}(L_B, L_A) &= \cos(\text{attn}(Q_B, K_B, V_B), \text{attn}(Q_B, K_A, V_A))\end{align}通过在预训练的U-Net或基于Transformer的模型中的注意力机制处理特征，AAS在注意力层中对齐两个密集的潜在表示，确保每个图像的特征既作为查询也作为键与另一图像的特征进行评估，从而提供了一种健壮的视觉相似性测量方法：\begin{equation}\text{Similarity}(L_A, L_B) = \text{AAS}(L_A, L_B) + \text{AAS}(L_B, L_A)\end{equation}这种方法不仅补偿了缺乏像素对齐的问题，还保留了特征空间的丰富性，提供了更准确地反映与人类视觉判断密切相符的感知相似性的方法。

\vspace{-0.3em}
\subsection{DiffSim Metric}
\vspace{-0.2em}
\label{sec:3}
\subsubsection{DiffSim in Self-attn Layer}
\label{sec:diffsim_self}
% 在海量图像文本对上预训练的stable diffusion unet是出色的视觉特征提取器，reference only方法直接将参考图像输入unet并将自注意力层中参考图的K和V直接与去噪unet的自注意力层中的K和V相连，实现了一致性的图像variation。 类似的，人体驱动任务中animate anyone, magicanimate等将unet作为提取参考图像细节信息的ReferenceNet, 并将ReferenceNet和去噪Unet的自注意力层相连进行条件信息的注入。同样的做法还被应用于人脸驱动和和Image2Video 。

% 在上述方法中，自注意力层中特征的嵌入可以实现外观一致性的图像或视频的生成，因此我们认为unet自注意力层的特征可以反应图像外观的一致性。我们提出了DiffSim的自注意力层实现。具体来说，我们计算


The pre-trained Stable Diffusion U-Net, extensively trained on massive image-text pairs, excels as a visual feature extractor. The reference only \citep{referenceonly} approach inputs reference images directly into the U-Net, connecting the reference image's keys (K) and values (V) in the self-attention layers directly with those in the denoising U-Net's self-attention layers to achieve consistent image variations. Similarly, in human-driven tasks such as Animate Anyone and MagicAnimate \citep{magicanimate, animateanyone}, the U-Net serves as a ReferenceNet to extract detailed information from reference images, linking its self-attention layers with those of the denoising U-Net for injecting conditional information. This technique is also applied in face-driven tasks \citep{emo, echomimic, idanimator, x-portrait}, image customization generation \citep{referenceonly, stablemakeup, stablehair}, and Image2Video generation \citep{livephoto, i2vgen-xl}. 

In the aforementioned methods, the embedding of features in the self-attention layers enables the generation of images or videos with appearance consistency. Thus, we posit that the features in the U-Net's self-attention layers can reflect the consistency of image appearance. We propose an implementation of the self-attention layers in DiffSim. We caculate:
\begin{equation}
\begin{aligned}
\text{DiffSim}(I_A, I_B, n, t) &= \frac{1}{2} \left( \text{AAS}(z_{t, \text{self}, n}^A , z_{t, \text{self}, n}^B ) \right.  \\
&\quad \left. + \text{AAS}(z_{t, \text{self}, n}^B , z_{t, \text{self}, n}^A ) \right),
\end{aligned}
\end{equation}
where \(z_{t, \text{self}, n}^A\) and \(z_{t, \text{self}, n}^B\) denote the latent representations of images \(I_A\) and \(I_B\) within the \(n\)-th self-attention layer of the U-Net at denoising timestep \(t\), respectively.


\begin{figure*}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{sec/Image/Bench2.pdf}
    \caption{To evaluate style similarity and instance-level similarity, we introduced the Sref bench and IP bench. The Sref dataset contains 508 styles, each generated by Midjourney's sref mode and handpicked by human artists, represented through four different thematic reference images. The IP dataset includes a set of 299 IPs comprising highly similar images along with variants that gradually decrease in similarity.}
    \label{bench}
\end{figure*}


% 为了评估风格相似性和instance-level similarity， 我们提出了Sref dataset 和 IP dataset。Sref dataset包含508种风格，每种风格都是由Midjourney的sref模式生成然后人类艺术家手工挑选，并通过四张不同主题的参考图片来展示。IP dataset 包含299个IP 的一组高度相似的图像，和其相似度逐渐降低的变体。

\vspace{-0.6em}
\subsubsection{DiffSim in Cross-attn Layer}
\vspace{-0.2em}
The Stable diffusion enhances text-to-image generation by integrating text embeddings as conditions within its cross-attention layers. Prior studies like Custom Diffusion have highlighted the pivotal role of these layers in learning customized model concepts, demonstrating that new concepts can be learned through mere fine-tuning of these layers. Given this context, we explored the potential of cross-attention layer features to assess image similarity. However, traditionally, cross-attention layers only support the calculation of attention between image latents and text embeddings. To extend their capability, we employed IP-Adapter Plus, which utilizes patch features from the CLIP image encoder and increases the number of IP tokens to 16, injecting these tokens into the cross-attention layers of Unet. This setup facilitates a more nuanced computation of attention that involves interaction between image latents and enhanced IP tokens.

We designed the structure illustrated in Figure ~\ref{fig:method}, where Image \(I_A\) and Image \(I_B\) are input into IP-Adapter Plus and the denoising Unet, respectively. The attention-based similarity scores are then computed by comparing the latents of one image to the IP tokens derived from the other, and vice versa. Specifically, we calculate:
\begin{equation}
\begin{aligned}
\text{DiffSim}(I_A, I_B, n, t) &= \frac{1}{2} \left( \text{AAS}(z_{t, \text{cross}, n}^A , IP_B) \right. \\
&\quad \quad \left. + z_{t, \text{cross}, n}^B, IP_A) \right),
\end{aligned}
\end{equation}
where \(z_{t, \text{cross}, n}^A\) and \(z_{t, \text{cross}, n}^B\) denote the latent representations of Images \(I_A\) and \(I_B\) within the \(n\)-th cross-attention layer of the U-Net at denoising timestep \(t\), respectively. Similarly, \(IP_A\) and \(IP_B\) represent the IP tokens associated with Images \(I_A\) and \(I_B\), respectively.


\vspace{-0.3em}
\subsubsection{DiffSim Adaptation to Various Frameworks}
% DiffSim的方法具有广泛的适用性，可以通过计算注意力层中特征相似性来分析两张图像的特征。我们已将DiffSim方法扩展应用于CLIP Image Encoder和DINO v2架构。CLIP通过对比学习训练图像和文本编码器，以理解图像与文本之间的关系，并最大化匹配图文对的相似性，通常采用Vision Transformer或ResNet作为图像编码器。DINO采用自监督方式，通过教师-学生网络架构，其中两者均使用Vision Transformer，学生网络通过模仿经数据增强的输入和教师网络的输出来学习视觉表示，教师网络则通过指数移动平均（EMA）进行更新。在特定自注意力层上，我们计算图像相似度，开发了新的指标CLIP Cross-SiM和DINO v2 Cross-Sim来评估相似性。

The DiffSim method is widely applicable and allows for the analysis of image features by computing feature similarity in the attention layers. We have extended the DiffSim approach to the CLIP Image Encoder and DINO v2 architectures. CLIP trains image and text encoders through contrastive learning to understand the relationship between images and text, aiming to maximize the similarity of matching image-text pairs, typically using Vision Transformer or ResNet as the image encoder. DINO operates in a self-supervised manner with a teacher-student network architecture, both utilizing Vision Transformers. The student network learns visual representations by mimicking the output of the teacher network, which has been augmented with random data transformations. The teacher network is updated through exponential moving average (EMA). For specific self-attention layers in the CLIP and DINO v2 models, we calculate AAS and introduce new metrics, CLIP AAS and DINO v2 AAS.

\vspace{-0.3em}
\subsection{Benchmark We Propose}
\vspace{-0.2em}
\label{sec:4}
\subsubsection{Sref Bench} Style is subjective, thus an effective style similarity metric should align with human perceptions and definitions of style. Therefore, we have collected 508 styles, each handpicked by human artists and featuring four thematically distinct reference images, created using Midjourney's Sref mode. Midjourney's style reference feature allows users to guide the style or aesthetic of generated images by using external pictures or style seeds in their prompts. Figure. \ref{bench} shows some examples in our benchmark.

% 风格本质上是主观的，因此一个好的风格相似度评估指标应当与人类对风格的感知和定义保持一致。为此，我们在网站上收集了508个人类艺术家精选的风格，每个风格包含四张题材不同的参考图像， 由Midjourney 的Sref模式创建。 Midjourney 的样式参考允许用户通过在提示中使用外部图片或风格种子作为参考来指导 Midjourney 生成的图像的风格或美感。

\vspace{-0.4em}
\subsubsection{IP Bench}
\vspace{-0.2em}
Instance-level consistency is one of the primary tasks in customized generation. However, there is a lack of high-quality benchmarks for assessing character consistency. We have collected images of 299 IP characters and used advanced Flux models \cite{flux} and the IP-Adapter to create several variants of each character with different consistency weights.

% 角色一致性是客制化生成的最要任务之一，然而角色一致性的评估缺乏优质的Benchmark。 我们收集了300个IP角色形象，基于先进的Flux模型和IP-Adapter制作每个形象在不同一致性权重下的的若干变体。


